MLLM-Tool: A Multimodal Large Language Model For Tool Agent Learning

Recently, the astonishing performance of large language models (LLMs) in natural language comprehension and generation tasks triggered lots of exploration of using them as central controllers to build agent systems. Multiple studies focus on bridging the LLMs to external tools to extend the application scenarios. However, the current LLMs' ability to perceive tool use is limited to a single text query, which may result in ambiguity in understanding the users' real intentions. LLMs are expected to eliminate that by perceiving the information in the visual- or auditory-grounded instructions. Therefore, in this paper, we propose MLLM-Tool, a system incorporating open-source LLMs and multi-modal encoders so that the learned LLMs can be conscious of multi-modal input instruction and then select the function-matched tool correctly. To facilitate the evaluation of the model's capability, we collect a dataset featuring multi-modal input tools from HuggingFace. Another essential feature of our dataset is that it also contains multiple potential choices for the same instruction due to the existence of identical functions and synonymous functions, which provides more potential solutions for the same query. The experiments reveal that our MLLM-Tool is capable of recommending appropriate tools for multi-modal instructions. Codes and data are available at https://github.com/MLLM-Tool/MLLM-Tool.

==> sec/7_limitation.tex <==
\section{Limitations}

Limited by the computation resources, MLLM-Tool now only supports single-turn conversations and independent multi-turn conversations. Since we directly perceive the content across multi-modal, enabling multi-turn conversations involves encoding the input and output of each modality for every turn, which brings more challenges, including insufficient window size to process and low overall encoding efficiency. Also, although we currently focus on API-type prediction, as predicting the correct API remains a complex task and current performance in this area is suboptimal, the collected dataset provides additional valuable information for the community to utilize.



==> tab/basic.tex <==
\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{cccc}
\hline
Images & Videos & Audios & Total\\ \hline
3798   & 103   & 726  &  4627\\ \hline
\end{tabular}
\caption{Multi-modal instruction-answer pairs.}
\label{tab:basic_table}
\end{table}

==> tab/combined.tex <==
% Table generated by Excel2LaTeX from sheet 'combined'
\begin{table}[htbp]
\renewcommand{\arraystretch}{1.1}
\resizebox{1\columnwidth}{!}{
    \begin{tabular}{cccc}
    \hline
    LLM  & Acc $\uparrow$ & Hallu $\downarrow$  & Format Acc$\uparrow$ \\
    \hline
    Vicuna-7B (2epochs) & 73.30  & 5.88  & 100.00  \\
    Llama-7B (2epochs) & 70.13  & 4.59  & 100.00  \\
    Llama2-7B (2epochs) & 70.21  & 4.76  & 100.00  \\
    Llama2-Chat-7B (2epochs) & 72.80  & 4.80  & 100.00  \\
    \hline
    Vicuna-7B (5epochs) & 83.15  & 1.63  & 100.00  \\
    Llama-7B (5epochs) & \textbf{84.48}  & \textbf{0.58}  & 100.00  \\
    Llama2-7B (5epochs) & 80.68  & 1.96  & 100.00  \\
    Llama2-Chat-7B (5epochs) & \uline{83.60}  & \uline{1.34}  & 100.00  \\
    \hline
    \end{tabular}}%
    \centering
  \caption{Main experiments of Tool-LMM. We present the performance of four large language models trained for two epochs and five epochs. We show the best score in bold and the second best underline.}
  \label{tab:combined}%
\end{table}%




% % Table generated by Excel2LaTeX from sheet 'combined'
% \begin{table}[htbp]
% \resizebox{1\columnwidth}{!}
% {
%     \begin{tabular}{cccc}
%     \hline
%     LLM  & Accu $\uparrow$ & hallu $\downarrow$  & Format Acc$\uparrow$ \\
%     \hline
%     Llama-7B (2epochs) & 70.13  & 4.59  & 100.00  \\
%     Llama2-7B (2epochs) & 70.21  & 4.76  & 100.00  \\
%     Llama2-Chat-7B (2epochs) & 72.80  & 4.80  & 100.00  \\
%     Vicuna-7B (2epochs) & 73.30  & 5.88  & 100.00  \\
%     Llama2-7B (5epochs) & 80.68  & 1.96  & 100.00  \\
%     Vicuna-7B (5epochs) & 83.15  & 1.63  & 100.00  \\
%     Llama2-Chat-7B (5epochs) & 83.60  & 1.34  & 100.00  \\
%     Llama-7B (5epochs) & \textbf{84.48}  & \textbf{0.58}  & 100.00  \\
%     \hline
%     \end{tabular}}%
%     \centering
%   \caption{Main experiments of ToolLMM. We present the performance of four large language models trained for two epochs and five epochs.}
%   \label{tab:combined}%
% \end{table}%





==> tab/modality.tex <==
% \begin{table*}[htbp]
% \centering
% \resizebox{2\columnwidth}{!}{
% \begin{tabular}{c c c c c c c c c}
% \hline
% \multirow{2}{*}{\textbf{Model}}& \multicolumn{2}{c}{\textbf{Video}} & \multicolumn{2}{c}{\textbf{Audio}} & \multicolumn{2}{c}{\textbf{Image}} & \multicolumn{2}{c}{\textbf{Text}}\\ 
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
% & Accuracy & Hall & Accuracy & Hall & Accuracy & Hall & Accuracy & Hall    \\ \hline
% Vicuna7b          & 85.71~            & 0.0000~ & 91.46~            & 0.6097~ & 92.76~            & 0.0000~ & 84.92~   & 0.0689~ \\
% LLaMa7b           & 71.43~            & 0.0000~ & 89.63~            & 0.0000~ & 93.16~            & 0.1316~ & 85.67~   & 0.2066~ \\
% LLaMa27b          & 80.95~            & 0.0000~ & 93.29~            & 0.0000~ & 91.71~            & 0.0000~ & 85.47~   & 0.0689~ \\
% LLaMa2chat7b    & 71.43~            & 0.0000~ & 90.85~            & 0.0000~ & 93.68~            & 0.0000~ & 85.95~   & 0.2066~ \\
% \hline
% \end{tabular}}
% \caption{Modality}
% \label{tab:modality}
% \end{table*}

% Table generated by Excel2LaTeX from sheet 'Modality'


\begin{table*}[t]
  \centering
  \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{ccccccccc}
    \hline
    \multirow{2}{*}{Model} & \multicolumn{2}{c}{Video} & \multicolumn{2}{c}{Audio} & \multicolumn{2}{c}{Image} & \multicolumn{2}{c}{Text}\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& Acc$\uparrow$ & Hallu$\downarrow$  & Acc$\uparrow$ & Hallu$\downarrow$  & Acc$\uparrow$ & Hallu$\downarrow$  & Acc$\uparrow$ & Hallu$\downarrow$\\
\hline
    Vicuna-7B (2epochs) & \uline{85.71}  & 0.00  & 91.46  & 0.00  & 71.84  & 8.42  & 71.83  & 5.30  \\
    Llama-7B (2epochs) & 66.67  & 0.00  & 88.41  & 0.61  & 62.63  & 2.11  & 72.04  & 6.40  \\
    Llama2-7B (2epochs) & \uline{85.71}  & 0.00  & 88.41  & 2.44  & 65.66  & 1.05  & 70.32  & 7.02  \\
    Llama2-Chat-7B (2epochs) & \textbf{90.48 } & 0.00  & 85.37  & 1.22  & 72.89  & 3.55  & 71.07  & 5.92  \\
    \hline
    Vicuna-7B (5epochs) & 71.43  & 0.00  & \textbf{93.29 } & 0.00  & \textbf{88.95 } & 0.53  & 79.13  & 2.41  \\
    Llama-7B (5epochs) & 76.19  & 0.00  & 89.02  & 0.00  & \uline{87.24}  & 0.26  & \textbf{82.64 } & 0.83  \\
    Llama2-7B (5epochs) & 80.95  & 0.00  & \textbf{93.29 } & 0.00  & 83.82  & 0.39  & 77.62  & 3.03  \\
    Llama2-Chat-7B (5epochs) & 80.95  & 0.00  & \uline{92.07}  & 0.00  & 86.45  & 1.84  & \uline{81.20}  & 1.24  \\
    \hline
    \end{tabular}%
    }
  \caption{Evaluating on four individual modality subsets.}
  \label{tab:modality}%
\end{table*}%

==> tab/ndcg.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
    \begin{tabular}{ccc}
    \hline
    \multicolumn{1}{l}{NDCG@1} & \multicolumn{1}{l}{NDCG@3} & \multicolumn{1}{l}{NDCG@5} \\
    \hline
    0.75  & 0.76  & 0.77  \\
    \hline
    \end{tabular}%
  \caption{NDCG}
  \label{tab:ndcg}%
\end{table}%


==> tab/one2mul.tex <==
% \begin{table}[htbp]
% \centering
% \begin{tabular}{l l l l l l l l l}
% \hline
% \multirow{2}{*}{\textbf{Model}}& \multicolumn{2}{c}{\textbf{One2Mul}} & \multicolumn{2}{c}{\textbf{One2One}}\\ 
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% & Accuracy & Hall & Accuracy & Hall\\ \hline
% Vicuna7b          & 77.11~            & 0.2915~                & 92.17~            & 0.0000~                 \\
% LLaMa7b           & 78.28~            & 0.4373~                & 92.17~            & 0.0584~                 \\
% LLaMa27b          & 77.99~            & 0.2915~                & 91.93~            & 0.0584~                 \\
% LLaMa2chat7b    & 79.59~            & 0.2915~                & 92.23~            & 0.0584~                 \\

% \hline
% \end{tabular}
% \caption{One2Mul}
% \label{tab:one2mul}
% \end{table}

% Table generated by Excel2LaTeX from sheet 'One2Mul'
\begin{table}[h]
  \centering
  \renewcommand{\arraystretch}{1.1}
  \resizebox{1\columnwidth}{!}{
    \begin{tabular}{ccccc}
    \hline
    \multirow{2}{*}{Model} & \multicolumn{2}{c}{one-to-one} & \multicolumn{2}{c}{one-to-many}\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}          & Acc$\uparrow$ & \multicolumn{1}{c}{Hallu$\downarrow$} & Acc$\uparrow$ & Hallu$\downarrow$\\
    \hline
    Vicuna-7B (2epochs) & 42.42  & 14.72  & 85.68  & 2.34  \\
    Llama-7B (2epochs) & 43.44  & 9.18  & 80.83  & 2.75  \\
    Llama2-7B (2epochs) & 40.52  & 10.35  & 82.12  & 2.51  \\
    Llama2-Chat-7B (2epochs) & 47.67  & 8.16  & 82.88  & 3.45  \\
    \hline
    Vicuna-7B (5epochs) & 66.03  & 3.35  & \uline{90.01}  & 0.94  \\
    Llama-7B (5epochs) & \uline{69.24}  & 1.31  & \textbf{90.59 } & 0.29  \\
    Llama2-7B (5epochs) & 63.12  & 3.64  & 87.73  & 1.29  \\
    Llama2-Chat-7B (5epochs) & \textbf{70.99 } & 2.33  & 88.66  & 0.94  \\
    \hline
    \end{tabular}}%
  \label{tab:one2mul}%
  \caption{The test set is divided into one-to-one and one-to-many based on how many APIs can be employed to tackle with the instruction. we illustrate the model's performance on two subsets.}
\end{table}%



